Identifying Relevant Information Cues for Vulnerability Assessment Using CVSS

The assessment of new vulnerabilities is an activity that accounts for information from several data sources and produces a `severity' score for the vulnerability. The Common Vulnerability Scoring System (\CVSS) is the reference standard for this assessment. Yet, no guidance currently exists on \emph{which information} aids a correct assessment and should therefore be considered. In this paper we address this problem by evaluating which information cues increase (or decrease) assessment accuracy. We devise a block design experiment with 67 software engineering students with varying vulnerability information and measure scoring accuracy under different information sets. We find that baseline vulnerability descriptions provided by standard vulnerability sources provide only part of the information needed to achieve an accurate vulnerability assessment. Further, we find that additional information on \texttt{assets}, \texttt{attacks}, and \texttt{vulnerability type} contributes in increasing the accuracy of the assessment; conversely, information on \texttt{known threats} misleads the assessor and decreases assessment accuracy and should be avoided when assessing vulnerabilities. These results go in the direction of formalizing the vulnerability communication to, for example, fully automate security assessments.

==> conclusion.tex <==
\noteKristian{ Summary of the rest }

\noteKristian{ The outcome should provide a list of recommendations for designers of CVSS and for software engineers on what the metrics helps them}

\noteKristian{ The following has to be adapted according to our final RESULTS section }

Based on our findings, we make the following recommendations to the CVSS designers:

%
\begin{itemize}
\item To avoid user frustration, the following metrics should be improved \dots
\item For systems were security is not a prime issue \dots
\item For systems were the knowledge of users of concepts such as 
\item The safest way for ensuring the quality of a vulnerability description
\end{itemize}


Based on our findings, we make the following recommendations for software engineers:

%
\begin{itemize}
\item Check the vulnerably for  \dots
\item What does the impact mean for your assets  \dots
\item For systems were security is a prime concern \dots
\item The safest way to assess software components is \dots
\end{itemize}

==> validity.tex <==
\noteHenning{In the whole paper: Check again: measure (German: Massnahme) != measurement != metric}
\noteHenning{In this section: There is a lot of defending and argueing going on. Let's just name the facts
\noteLuca{I don't know where this section comes from but it seems to me it's from another paper. It's to be rewritten completely.}}

We discuss the threats to validity using the four validity classes proposed by Wohlin et al. \cite{Wohlin2012}. 

%construction validity
%threats to the generalization of results to a theory
%such as only one method used
\emph{Construct validity} The measurements of the experiment include a scoring system for vulnerabilities and an evaluation of the number of errors in relation to a gold standard. The CVSS vulnerability scoring is an internationally established method to assess the impact a vulnerability can have and so far no significant alternative exist. Therefore, we believe this measure to be appropriate for our study. 
\noteHenning{That's a weird argument. No alternative exists, therefore it's good? How about: It's established, therefore it's good? (throw away the alternative part)}
In addition, this measurement does not provide insights into the mental process behind a vulnerability rating. Future studies using detailed interviews or even clinical studies observing engineers in the wild, on how engineers handle and address vulnerability issues may provide additional insights. 

%conclusion validity
%problems with the experiment that lead to wrong conclusions
%such as low statistical power or a high error rate
%Are the measures made  really representative of applicability, or could there be other better measures.
 \emph{Conclusion validity} 
 The experiment was conducted on paper. On this paper, we outlined each step of the method provided some examples. The examples were perceived and applied well to a different context by some participants, while others stated that they would like more and different examples. 
 \noteHenning{How do we know? Did we ask? Study design?}
 \noteHenning{What does applied well to... mean?}
 We decided not to put too many examples in order to avoid lengthy texts. Moreover, the experiment was done on paper, but digitalised into an excel file afterwards. Two independent people validated the digitalisation. Moreover, the participants were in all in one room during the scoring. We asked them not to talk to each other during the lab and supervised them, but we had no means to ensure this did not happen anywhere during the experiment. 
 \noteHenning{Could we state: "We did not observe any irregularities." ? Then we can remove the rest of the argumentation.}
 We observed the over 100 students with 5 people in different corners of the room and believe this reasonable coverage shall have minimised issues arising from this problem. 

%internal validity
 %influences on the independent variables 
% with respect to causality
  %problems with incorrect sampling could be an issue here
  \emph{Internal validity} 
  \noteHenning{Next one is external.}
A threat to the external validity is that we conducted the experiment with students instead of practitioners from industry. However, the sample was taken in a specific master programs for  software engineering related disciplines and many students have had years of experience working in the automotive domain. It is a particular challenge to gather a large sample group of this type, which is highly representative of the target audience and we admit that practitioners would improve the study, but our precise sampling let us say with confidence that we believe our results do have value. 
\noteHenning{The last two sentences sound like defending and they are unsubstantiated anyways, let's just remove them. The next sentence is way better defending.}
 We did analyse the knowledge of the students in terms of software engineering and security to describe their education via self assessment and asked them multiple choice questions to provide a proof of the self assessment. This helped to describe the sample in adequate detail. We argue the our master students are few month or years ahead of a career in industry a provide sufficient similarity with junior engineers in their first month in a job. Furthermore, we argue that if our students can achieve a correct vulnerability scoring, their counterparts in industry could as well. This leaves the validity concern that the practitioner might be slightly better. 
%Moreover, our sample of over 100 students are close to junior practitioners that start in companies. 
Therefore, we are reasonably certain the results of this experiment provide reliable conclusions. 
 
  %external validity
 %influences on the independent variables with respect to causality
 %with regard to apply it in industry
 %timing of the experiment e.g. before deadline
\emph{External validity} 
 We had a single group of participants conducting the experiment that are students. We did analyse the knowledge of the students in terms of software engineering and security to describe their education via self assessment and asked them multiple choice questions to provide a proof of the self assessment. This helped to describe the sample in adequate detail. We argue the our master students are few month or years ahead of a career in industry a provide sufficient similarity with junior engineers in their first month in a job. Furthermore, we argue that if our students can achieve a correct vulnerability scoring, their counterparts in industry could as well. This leaves the validity concern that the practitioner might be slightly better. 

\noteHenning{In our passive voice paper, we argue: The first threat relates to the generalizability of results to industrial practices, since participants of the experiment were students. The use of stu- dents as study subjects has been longly discussed in the soft- ware engineering literature and in general considered as suitable under certain conditions, based on generally accepted criteria for validity evaluation of empirical studies [6]. Rune- son [13] observed that graduate level students are feasible subjects for revealing improvement trends: since the focus in our study was a comparison and not to find an absolute level of improvements, according to [13] the use of students in our case is suitable. In addition, a study on requirements prioritisation [2] showed that experience and commitment are important factors when using students as study sub- jects: we balanced this threat by letting the participation of students voluntary and by ensuring an adequate level of experience and skills of participants. Finally, we used re- quirements from real industrial projects.
[6] M. Ho ̈st, B. Regnell, and C. Wohlin. Using students as subjects - a comparative study of students and professionals in lead-time impact assessment. Empirical Softw. Eng., 2000.
[2] P. Berander. Using students as subjects in requirements prioritization. In ISESE, Aug 2004.
[13] P. Runeson. Using Students as Experiment Subjects - An Analysis on Graduate and Freshmen Student Data. In EASE, 2003.
}
 

